Black-Box Policy Search with Probabilistic Programs

In this work, we explore how probabilistic programs can be used to represent policies in sequential decision problems. In this formulation, a probabilistic program is a black-box stochastic simulator for both the problem domain and the agent. We relate classic policy gradient techniques to recently introduced black-box variational methods which generalize to probabilistic program inference. We present case studies in the Canadian traveler problem, Rock Sample, and a benchmark for optimal diagnosis inspired by Guess Who. Each study illustrates how programs can efficiently represent policies using moderate numbers of parameters.

==> Makefile <==
all: mdpp.pdf mdpp.aux

PDFLATEX=pdflatex -shell-escape

%.aux: %.tex
	$(PDFLATEX) ${basename $<}

%.bbl: %.aux
	bibtex ${basename $<}

%.pdf: %.bbl
	$(PDFLATEX) ${basename $<}
	$(PDFLATEX) ${basename $<}

mdpp.pdf: mdpp.tex \
	mdpp.bib


clean:
	rm -f *.aux *.log *.bbl *.blg 

distclean: clean
	rm -f mdpp.pdf


==> related.tex <==
% !TEX root =  mdpp.tex

\subsection{Planning and Control as Inference}

Our formulation of policy search as expectation maximization in probabilistic programs fits into a long history of approaches that frame planning and control problems as inference. Path integral methods \cite[]{kappen_jsmtm_2005,kappen_cbns_2007,broek_jair_2008,todorov_nips_2009,todorov_pnas_2009,kappen_ml_2012} express the expected cost-to-go as a KL-divergence between a posterior, controlled, distribution on $x_{1:T}$ and a distribution defined as the product of the prior, uncontrolled, dynamics and the exponent of the reward. Minimization of this KL divergence is then equivalent to minimization of the expected cost-to-go. In the context of these types of approaches, minimization of the expected exponentially weighted cost-to-go is known as risk-sensitive optimal control \cite[]{vandenbroek_uai_2010}. Path integral approaches have been applied to reinforcement learning problems in a number of studies \cite[]{theodorou_aistats_2010,theodorou_cdc_2012,azar_jmlr_2012}. 

Related approaches \cite[]{rawlik_nips_2010,rawlik_rss_2012} minimize the KL divergence between the  distribution on trajectories $\t$ induced by a stochastic policy $\pi$ relative to that induced by a an exponentially weighted posterior distribution with policy $\pi_0$. This is equivalent to a optimal control problem in which the reward is discounted by the log probability of the actions under $\pi_0$. Iterative solution, in which each $\pi_i$ is obtained by KL minimization relative to the posterior induced by $\pi_{i-1}$, converges to the optimal policy in this setting, which is consistent with our observation that expectation maximization is equivalent to maximization of the expected reward. 

The use of variational inference in reinforcement learning problems has also been explored in a number of ways. When the reward is non-negative, variational Bayes and expectation propagation can be used to approximate a posterior in a (non-exponentiated) reward weighted model \cite[]{furmston_icml_2010}. The exponentiated reward case has similarly been considered \cite[]{neumann_icml_2011}. In this setting, it has been observed that minimization of the M-projection (i.e. the KL divergence between posterior and variational distribution, as used in expectation propagation) instead of the I-projection (i.e. the KL divergence between the variational distribution distribution and the posterior) leads to an objective that is equivalent to that used in Monte-Carlo EM approaches \cite[]{kober_ml_2011,vlassis_ar_2009}. As noted, the variant of BBVI used here is closely related to the one proposed by \cite[]{wingate_arxiv_2013} for probabilistic programs.

\subsection{Policies as Programs}



